ManiWAV: Learning Robot Manipulation from In-the-Wild Audio-Visual Data

Audio signals provide rich information for the robot interaction and object properties through contact. This information can surprisingly ease the learning of contact-rich robot manipulation skills, especially when the visual information alone is ambiguous or incomplete. However, the usage of audio data in robot manipulation has been constrained to teleoperated demonstrations collected by either attaching a microphone to the robot or object, which significantly limits its usage in robot learning pipelines. In this work, we introduce ManiWAV: an 'ear-in-hand' data collection device to collect in-the-wild human demonstrations with synchronous audio and visual feedback, and a corresponding policy interface to learn robot manipulation policy directly from the demonstrations. We demonstrate the capabilities of our system through four contact-rich manipulation tasks that require either passively sensing the contact events and modes, or actively sensing the object surface materials and states. In addition, we show that our system can generalize to unseen in-the-wild environments by learning from diverse in-the-wild human demonstrations.

==> text/old_text/introduction.tex <==
\section{Introduction}
\label{sec:intro}
% \zeyi{good contact is key to manipulation success - visuomotor policy fail at contact-rich tasks - we need to better utilize contact information, this requires improvement in both hardware and algorithm front - hardware front: tactile - contact mic, lab teleop - in-the-wild collection, algo front: modality encoding and fusion strategy, deal with noise / ood scenarios - we propose xxx, summarize our pipeline and contributions}

When interacting with objects in daily life, we are constantly making contacts (e.g. grasping a cup, wiping table). Making good contact is a key to manipulation success. Most manipulation tasks require the right amount and direction of force to be exerted on the actuated object (e.g. screw a bottle cap) and knowing when to switch between different contact events (e.g. wiping). We can also infer object physical state or material property through contacts, which guides decision making in the manipulation process.

Recently, end-to-end behavior cloning models such as Diffusion Policy \cite{chi2023diffusion} and ACT \cite{zhao2023learning} have demonstrated strong capability in learning versatile robot manipulation skills from human demonstrations. However, these models only consider visual observations and may fall short in contact-rich manipulation tasks due to occlusion or visual ambiguity.

So how can we better incorporate contact information for learning robot manipulation policies? We think the solutions come from both the hardware and algorithm.

On the hardware front, prior works have shown that tactile sensors are able to provide rich contact information for many robot manipulation tasks. However, tactile sensors are limited by 1) need to make direct contact with object; 2) expensive and fragile, which limit the scale of data; 3) require separate streaming, which limit data collection to teleoperation in lab. We identify sounds captured by contact microphone as an alternative to represent contact information, see figure 1. 1) it does not require direct contact with the object as vibrations can be transmitted through all medium 2) it is cheap (\$10) and robust 3) the information can be easily streamed and stored with vision in video format. Given these nice properties of contact microphone, we propose to use a low-cost, scalable in-the-wild data collection device to collect vision and contact sound data.

% First of all, it's the scarcity of data.
% There's no in-the-wild robot collection data device that simultaneously collects vision and sound data. Most focus on vision data~\cite{padalkar2023open, chi2024universal, khazatsky2024droid}. Current setups that collect audio data are limited to teleoperation in lab with fixed microphone locations~\cite{fang2023rh20t, li2022see}. In addition, audio data are subject to background noises. So we propose a in-the-wild data collection device.

On the algorithm front, one key challenge is the audio domain gap between human collected data and actual robot deployment due to robot motor noises and out-of-distribution sounds during robot execution. Another challenge is how to effectively fuse the vision and audio modalities as at different stages of the task, one modality might at higher importance than the other. We propose an audio data augmentation strategy together with a sensory fusion model to learn audiovisual representation for downstream robotic tasks. \zeyi{Previous method also uses MLP as the policy head, we use diffusion policy that's better suited to learn the multi-modality in human demonstrations}

% On the method front, it is yet unclear whether such human collected data can be used to train a robot policy that is directly deployable on a real robot. Some challenges are domain gap coming from human demonstration and real time robot deployment. Effective encoding and fusion of the modalities are also important.

In summary, we propose a complete pipeline to learn robot manipulation skills from human collected vision and sound information. Our system includes:
\begin{itemize}
    \item A in-the-wild data collection device that collects synchronized vision and contact sound data.
    \item An end-to-end learning pipeline that generates deployable robot policy directly from human collected vision and sound data.
    \item A set of experiments that demonstrate the capability and use cases of our system.
\end{itemize}



